The Effects of Computational Resources on Flaky Tests

Flaky tests are tests that nondeterministically pass and fail in unchanged code. These tests can be detrimental to developers' productivity. Particularly when tests run in continuous integration environments, the tests may be competing for access to limited computational resources (CPUs, memory etc.), and we hypothesize that resource (in)availability may be a significant factor in the failure rate of flaky tests. We present the first assessment of the impact that computational resources have on flaky tests, including a total of 52 projects written in Java, JavaScript and Python, and 27 different resource configurations. Using a rigorous statistical methodology, we determine which tests are RAFT (Resource-Affected Flaky Tests). We find that 46.5% of the flaky tests in our dataset are RAFT, indicating that a substantial proportion of flaky-test failures can be avoided by adjusting the resources available when running tests. We report RAFTs and configurations to avoid them to developers, and received interest to either fix the RAFTs or to improve the specifications of the projects so that tests would be run only in configurations that are unlikely to encounter RAFT failures. Our results also have implications for researchers attempting to detect flaky tests, e.g., reducing the resources available when running tests is a cost-effective approach to detect more flaky failures.

==> old/introduction.tex <==
Flaky tests are tests that can pass and fail in repeated executions without changes to the test code or the code under test (CUT). Flaky tests significantly affect developer productivity. In a continuous integration environment, test failures require developers to investigate root causes and repair corresponding code.
The detrimental effects of flaky tests have been reported as a major issue by major software companies~\Fix{cite} and triggered intensive research over the past years~\Fix{cite}, mostly pertaining to detecting and repairing flaky tests of certain types, such as implementation dependent tests \cite{Shi2016GLM} or order dependent tests \cite{Zhang2014JWMLEN, Lam2019OSMX, Shi2019LOXM, Wei2021YXML}.

% \Fix{add more here}

% in both the scientific literature and practical approaches for coping with flaky tests 
An aspect that has remained largely unexplored in the literature is the impact of resource availability (or lack thereof) on flaky test failures. Intuitively, the unavailability of required computational resources, such as the CPU, main memory, network and disk I/O bandwidth, can lead to run time errors that affect test execution.
For instance, if CPU resources are unavailable, either due to test execution on a weakly equipped machine\MyComment{ or CPU contention in a multi-processing/multi-tenant setting}, implicit test assumptions on the latency of asynchronous operations may be violated and lead to test failures \cite{silva2020shake} ~\Mar{cite shaker and other work on UI test flakiness}.

Most existing approaches for flaky test detection rely on the re-execution of failing tests.
These approaches are not capable of detecting \emph{resource-affected flaky tests} (RAFT), unless the unavailable resources become available in between test repetitions.
While this may happen by chance, it is not an aspect that is controlled for in existing approaches.
Consequently, while RAFT may be detected by existing approaches by chance, they cannot be remediated as their root cause cannot be correctly identified.

In our study, we address this problem and provide, for the first time, empirical evidence for effects of resource unavailability on test results. 
While we find obvious violations of test assumptions, like in the examples provided above, we also identify a number of subtle dependencies on resource availability.
We propose two detection approaches for RAFT.
One approach (RAFT\textsubscript{\em di}) randomly injects delays by inserting sleep calls into test code.
The other approach (RAFT\textsubscript{\em th}) throttles resource access during test execution via Linux cgroups.

In this paper, we present initial evidence of platform-dependent flaky tests that exhibit significantly different failure rates depending on the hardware configuration they are run on.
More specifically, we demonstrate the effect of resource (un-)availability on flaky test failure rates.
We show that \emph{resource-affected flaky tests} (RAFT)\ldots\swnote{add results hint here}. 
This finding is of high practical relevance for regression tests that can run on different hardware configurations or on shared hardware with load that varies over time, which can both entail resource contention.
It also has strong implications for debugging flaky test failures, as debugging is commonly conducted on a \emph{different} machine than the machine on which the test failed in regression testing.
\Fix{See if this is true from results and revisit:} Furthermore, we show that increasing resources beyond a point has diminishing returns and there exists an optimal configuration which minimizes over cost and test flakiness.
This finding is of high practical relevance for cost optimization, as it hints towards thresholds for minimal resource allocation necessary to mitigate RAFT.

We devise and empirically assess two systematic approaches to increase the reproducibility of RAFT to help developers with their (a) detection, (b) debugging, and (c) effect forecasting for regression testing on a given platform.
Our results show that \ldots\swnote{add results summary here}

==> tables/buildsAndCosts.tex <==
\setlength{\tabcolsep}{3pt}
\caption{\label{lbl:rq3} How often does a build fail due to a flaky test, for each configuration? F is percentage of builds that failed. P is price per thousand runs.}
\jon{Note that we did not use fail-fast, make sure that this is addressed in the text}
\jon{2-4-23 confirmed we have everything that we should in this table. note: for failures here, we include ANY flaky test failure in the build, not just failures of RAFT tests... this seems to make sense}
\centering
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{0.1c/1GB} & \multicolumn{2}{c}{0.1c/2GB} & \multicolumn{2}{c}{0.25c/2GB} & \multicolumn{2}{c}{0.5c/2GB} & \multicolumn{2}{c}{0.5c/4GB} & \multicolumn{2}{c}{1c/4GB} & \multicolumn{2}{c}{1c/8GB} & \multicolumn{2}{c}{2c/4GB} & \multicolumn{2}{c}{2c/8GB} & \multicolumn{2}{c}{2c/16GB} & \multicolumn{2}{c}{4c/8GB} & \multicolumn{2}{c}{4c/16GB} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11} \cmidrule(l{3pt}r{3pt}){12-13} \cmidrule(l{3pt}r{3pt}){14-15} \cmidrule(l{3pt}r{3pt}){16-17} \cmidrule(l{3pt}r{3pt}){18-19} \cmidrule(l{3pt}r{3pt}){20-21} \cmidrule(l{3pt}r{3pt}){22-23} \cmidrule(l{3pt}r{3pt}){24-25}
 & F & P & F & P & F & P & F & P & F & P & F & P & F & P & F & P & F & P & F & P & F & P & F & P\\
\midrule
\cellcolor{gray!6}{assertj-core} & \cellcolor{gray!6}{76} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{67} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{19} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{9} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{9} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{10} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{11} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{10} & \cellcolor{gray!6}{\textbf{0.09}} & \cellcolor{gray!6}{\textbf{8}} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{14} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{11} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{11} & \cellcolor{gray!6}{0.19}\\
carbon-apimgt & 1 & \textbf{0.11} & \textbf{0} & 0.16 & \textbf{0} & \textbf{0.11} & \textbf{0} & \textbf{0.11} & \textbf{0} & 0.15 & \textbf{0} & 0.17 & \textbf{0} & 0.22 & \textbf{0} & 0.24 & \textbf{0} & 0.28 & \textbf{0} & 0.38 & \textbf{0} & 0.48 & \textbf{0} & 0.56\\
\cellcolor{gray!6}{commons-exec} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{\textbf{0.09}} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{3} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.29} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.37} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.45} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.55} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.72} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{1.11}\\
db-scheduler & 26 & 0.07 & 29 & 0.10 & 15 & \textbf{0.06} & 3 & \textbf{0.06} & 3 & 0.08 & \textbf{0} & 0.09 & \textbf{0} & 0.11 & \textbf{0} & 0.12 & \textbf{0} & 0.15 & \textbf{0} & 0.19 & \textbf{0} & 0.23 & \textbf{0} & 0.27\\
\cellcolor{gray!6}{delight-nashorn-sandbox} & \cellcolor{gray!6}{37} & \cellcolor{gray!6}{0.35} & \cellcolor{gray!6}{38} & \cellcolor{gray!6}{0.54} & \cellcolor{gray!6}{48} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{34} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{35} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{8} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{6} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.16}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.30} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.35}\\
elastic-job-lite & \textbf{0} & 0.28 & \textbf{0} & 0.42 & \textbf{0} & 0.25 & \textbf{0} & \textbf{0.24} & - & - & \textbf{0} & 0.29 & \textbf{0} & 0.38 & \textbf{0} & 0.49 & \textbf{0} & 0.49 & \textbf{0} & 0.65 & \textbf{0} & 0.97 & \textbf{0} & 0.89\\
\cellcolor{gray!6}{esper} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.06}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{7} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{6} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{5} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{6} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{9} & \cellcolor{gray!6}{0.19}\\
excelastic & 89 & 0.06 & 85 & 0.09 & \textbf{8} & 0.06 & 16 & \textbf{0.05} & 22 & 0.06 & 57 & 0.06 & 58 & 0.08 & 61 & 0.08 & 65 & 0.09 & 63 & 0.10 & 69 & 0.13 & 68 & 0.17\\
\cellcolor{gray!6}{fastjson} & \cellcolor{gray!6}{10} & \cellcolor{gray!6}{0.38} & \cellcolor{gray!6}{9} & \cellcolor{gray!6}{0.59} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.33} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{\textbf{0.27}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.35} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.36} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.31} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.36} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.47} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.69} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.72}\\
fluent-logger-java & 38 & \textbf{0.09} & 20 & 0.14 & \textbf{0} & 0.10 & \textbf{0} & 0.12 & \textbf{0} & 0.15 & \textbf{0} & 0.19 & \textbf{0} & 0.25 & \textbf{0} & 0.30 & \textbf{0} & 0.36 & \textbf{0} & 0.46 & \textbf{0} & 0.59 & \textbf{0} & 0.70\\
\cellcolor{gray!6}{handlebars.java} & \cellcolor{gray!6}{3} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{3} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{\textbf{0.07}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.17}\\
hector & 49 & 0.40 & 47 & 0.59 & 36 & 0.32 & 37 & \textbf{0.24} & 36 & 0.32 & 30 & 0.25 & 37 & 0.32 & \textbf{13} & 0.27 & 19 & 0.32 & 20 & 0.43 & 16 & 0.54 & 19 & 0.68\\
\cellcolor{gray!6}{http-request} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.03}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.03}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.03}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.08}\\
httpcore & 15 & 0.11 & 14 & 0.18 & 8 & 0.10 & 8 & \textbf{0.09} & 8 & 0.12 & 8 & 0.13 & 6 & 0.22 & \textbf{2} & 0.15 & 5 & 0.17 & 6 & 0.23 & 7 & 0.48 & 8 & 0.52\\
\cellcolor{gray!6}{hutool} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.03} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.03} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.02}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.06}\\
incubator-dubbo & - & - & - & - & \textbf{0} & 2.07 & 4 & \textbf{1.93} & 4 & 2.50 & 4 & 2.62 & 3 & 3.55 & 1 & 3.55 & 3 & 4.19 & 1 & 5.46 & 1 & 7.19 & 2 & 8.14\\
\cellcolor{gray!6}{java-websocket} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{3}} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{24} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{30} & \cellcolor{gray!6}{\textbf{0.07}} & \cellcolor{gray!6}{35} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{33} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{32} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{32} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{37} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{33} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{29} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{20} & \cellcolor{gray!6}{0.23}\\
logback & 37 & \textbf{0.21} & 41 & 0.36 & 16 & 0.45 & 14 & 0.59 & 10 & 0.91 & 13 & 1.04 & 12 & 1.44 & \textbf{2} & 1.67 & \textbf{2} & 2.61 & 4 & 3.09 & 3 & 3.83 & 4 & 5.19\\
\cellcolor{gray!6}{luwak} & \cellcolor{gray!6}{3} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.08}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.21}\\
ninja & \textbf{1} & 0.23 & 2 & 0.35 & 3 & 0.19 & 2 & \textbf{0.15} & 2 & 0.20 & 2 & 0.17 & 3 & 0.21 & \textbf{1} & 0.18 & 4 & 0.19 & 4 & 0.25 & 4 & 0.30 & 2 & 0.33\\
\cellcolor{gray!6}{noxy} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.39} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.16}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.16}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.30} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.37}\\
orbit & 36 & \textbf{0.22} & 37 & 0.35 & 24 & 0.26 & 12 & 0.27 & 16 & 0.35 & 13 & 0.43 & 12 & 0.56 & 8 & 0.65 & 8 & 0.77 & \textbf{5} & 0.99 & 7 & 1.28 & 8 & 1.50\\
\cellcolor{gray!6}{oryx} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.09}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.31} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.41} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.48} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.58}\\
riptide & \textbf{0} & 0.12 & \textbf{0} & 0.19 & \textbf{0} & 0.12 & 97 & \textbf{0.11} & 96 & 0.15 & 97 & 0.16 & 97 & 0.20 & \textbf{0} & 0.21 & 3 & 0.29 & \textbf{0} & 0.33 & \textbf{0} & 0.26 & \textbf{0} & 0.31\\
\cellcolor{gray!6}{rxjava2-extras} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.35} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.21}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.27} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.30} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.39} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.41} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.50} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.65} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.87} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.95}\\
spring-boot & - & - & \textbf{0} & 1.69 & \textbf{0} & 1.02 & \textbf{0} & \textbf{0.73} & 1 & 0.97 & 1 & 0.80 & \textbf{0} & 0.98 & \textbf{0} & 0.77 & \textbf{0} & 0.90 & \textbf{0} & 1.25 & \textbf{0} & 1.46 & \textbf{0} & 2.00\\
\cellcolor{gray!6}{timely} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.33} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{0.12}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{0.23}\\
undertow & - & - & \textbf{0} & 0.52 & \textbf{0} & 0.29 & \textbf{0} & \textbf{0.23} & \textbf{0} & 0.30 & \textbf{0} & 0.25 & \textbf{0} & 0.33 & \textbf{0} & 0.30 & \textbf{0} & 0.36 & \textbf{0} & 0.46 & \textbf{0} & 0.58 & 1 & 0.68\\
\cellcolor{gray!6}{wildfly} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{5.80} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3.74} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{3.01} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{3.81} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{\textbf{2.86}} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{3.32} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{4.35} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{5.38} & \cellcolor{gray!6}{\textbf{0}} & \cellcolor{gray!6}{6.58}\\
wro4j & - & - & - & - & - & - & - & - & \textbf{0} & 1.27 & 1 & 0.91 & 1 & 1.20 & 40 & \textbf{0.83} & 10 & 0.93 & 30 & 1.27 & 39 & 1.22 & 32 & 1.44\\
\cellcolor{gray!6}{yawp} & \cellcolor{gray!6}{15} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{18} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{3} & \cellcolor{gray!6}{\textbf{0.06}} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{3} & \cellcolor{gray!6}{\textbf{0.06}} & \cellcolor{gray!6}{5} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{6} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{5} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{8} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{8} & \cellcolor{gray!6}{0.16}\\
zxing & 10 & 0.67 & 7 & 0.90 & 7 & 0.50 & 8 & \textbf{0.38} & 8 & 0.49 & 8 & \textbf{0.38} & \textbf{6} & 0.49 & 8 & 0.56 & \textbf{6} & 0.66 & 9 & 0.86 & \textbf{6} & 1.12 & 7 & 1.32\\
\bottomrule
\end{tabular}

==> tables/detection-and-cost.tex <==
\setlength{\tabcolsep}{3pt}
\caption{\label{lbl:rq4}Number of flaky tests detected (T) and price per thousand runs for each of the projects in our dataset.}
    \jon{2-4-23 confirmed that we have all of the data in here, should be final table. note again, that for this RQ we are probably more interested in total number of flaky tests found, rather than just RAFT tests, so this shows all flakies found (not just RAFT)}
\centering
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{0.1c/1GB} & \multicolumn{2}{c}{0.1c/2GB} & \multicolumn{2}{c}{0.25c/2GB} & \multicolumn{2}{c}{0.5c/2GB} & \multicolumn{2}{c}{0.5c/4GB} & \multicolumn{2}{c}{1c/4GB} & \multicolumn{2}{c}{1c/8GB} & \multicolumn{2}{c}{2c/4GB} & \multicolumn{2}{c}{2c/8GB} & \multicolumn{2}{c}{2c/16GB} & \multicolumn{2}{c}{4c/8GB} & \multicolumn{2}{c}{4c/16GB} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9} \cmidrule(l{3pt}r{3pt}){10-11} \cmidrule(l{3pt}r{3pt}){12-13} \cmidrule(l{3pt}r{3pt}){14-15} \cmidrule(l{3pt}r{3pt}){16-17} \cmidrule(l{3pt}r{3pt}){18-19} \cmidrule(l{3pt}r{3pt}){20-21} \cmidrule(l{3pt}r{3pt}){22-23} \cmidrule(l{3pt}r{3pt}){24-25}
 & T & P & T & P & T & P & T & P & T & P & T & P & T & P & T & P & T & P & T & P & T & P & T & P\\
\midrule
\cellcolor{gray!6}{assertj-core} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{\textbf{3}} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.09}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.19}\\
carbon-apimgt & \textbf{1} & \textbf{0.11} & \textbf{1} & 0.16 & \textbf{1} & \textbf{0.11} & 0 & \textbf{0.11} & 0 & 0.15 & 0 & 0.17 & \textbf{1} & 0.22 & 0 & 0.24 & 0 & 0.28 & 0 & 0.38 & 0 & 0.48 & 0 & 0.56\\
\cellcolor{gray!6}{commons-exec} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{\textbf{0.09}} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.21} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.29} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.37} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.45} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.55} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.72} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.97} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{1.11}\\
db-scheduler & \textbf{6} & 0.07 & \textbf{6} & 0.10 & \textbf{6} & \textbf{0.06} & \textbf{6} & \textbf{0.06} & \textbf{6} & 0.08 & \textbf{6} & 0.09 & 5 & 0.11 & 5 & 0.12 & 5 & 0.15 & 5 & 0.19 & 5 & 0.23 & 5 & 0.27\\
\cellcolor{gray!6}{delight-nashorn-sandbox} & \cellcolor{gray!6}{25} & \cellcolor{gray!6}{0.35} & \cellcolor{gray!6}{\textbf{26}} & \cellcolor{gray!6}{0.54} & \cellcolor{gray!6}{8} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{7} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{7} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{4} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{6} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.16}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.25} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.30} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.35}\\
elastic-job-lite & \textbf{0} & 0.28 & \textbf{0} & 0.42 & \textbf{0} & 0.25 & \textbf{0} & \textbf{0.24} & - & - & \textbf{0} & 0.29 & \textbf{0} & 0.38 & \textbf{0} & 0.49 & \textbf{0} & 0.49 & \textbf{0} & 0.65 & \textbf{0} & 0.97 & \textbf{0} & 0.89\\
\cellcolor{gray!6}{esper} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{\textbf{0.06}} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.16} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.19}\\
excelastic & \textbf{2} & 0.06 & \textbf{2} & 0.09 & 1 & 0.06 & 1 & \textbf{0.05} & 1 & 0.06 & 1 & 0.06 & 1 & 0.08 & 1 & 0.08 & 1 & 0.09 & 1 & 0.10 & 1 & 0.13 & 1 & 0.17\\
\cellcolor{gray!6}{fastjson} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.38} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.59} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.33} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{\textbf{0.27}} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.35} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.28} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.36} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.31} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.36} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.47} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.69} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.72}\\
fluent-logger-java & \textbf{2} & \textbf{0.09} & \textbf{2} & 0.14 & 1 & 0.10 & 0 & 0.12 & 0 & 0.15 & 0 & 0.19 & 0 & 0.25 & 0 & 0.30 & 0 & 0.36 & 0 & 0.46 & 0 & 0.59 & 0 & 0.70\\
\cellcolor{gray!6}{handlebars.java} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{\textbf{0.07}} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.17}\\
hector & \textbf{2} & 0.40 & \textbf{2} & 0.59 & \textbf{2} & 0.32 & \textbf{2} & \textbf{0.24} & \textbf{2} & 0.32 & \textbf{2} & 0.25 & \textbf{2} & 0.32 & \textbf{2} & 0.27 & 1 & 0.32 & \textbf{2} & 0.43 & 1 & 0.54 & \textbf{2} & 0.68\\
\cellcolor{gray!6}{http-request} & \cellcolor{gray!6}{\textbf{6}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{6}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{5} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{6}} & \cellcolor{gray!6}{\textbf{0.03}} & \cellcolor{gray!6}{\textbf{6}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{5} & \cellcolor{gray!6}{\textbf{0.03}} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{\textbf{0.03}} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.08}\\
httpcore & 3 & 0.11 & \textbf{6} & 0.18 & 2 & 0.10 & \textbf{6} & \textbf{0.09} & 3 & 0.12 & 5 & 0.13 & 4 & 0.22 & 3 & 0.15 & 5 & 0.17 & 4 & 0.23 & 3 & 0.48 & 4 & 0.52\\
\cellcolor{gray!6}{hutool} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.06} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.03} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.03} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{\textbf{0.02}} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.04} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.05} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.06}\\
incubator-dubbo & - & - & - & - & \textbf{17} & 2.07 & 5 & \textbf{1.93} & 5 & 2.50 & 2 & 2.62 & 5 & 3.55 & 2 & 3.55 & 3 & 4.19 & 1 & 5.46 & 2 & 7.19 & 3 & 8.14\\
\cellcolor{gray!6}{java-websocket} & \cellcolor{gray!6}{33} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{\textbf{34}} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{33} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{32} & \cellcolor{gray!6}{\textbf{0.07}} & \cellcolor{gray!6}{31} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{28} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{29} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{23} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{23} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{26} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{23} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{22} & \cellcolor{gray!6}{0.23}\\
logback & \textbf{21} & \textbf{0.21} & 20 & 0.36 & 13 & 0.45 & 10 & 0.59 & 8 & 0.91 & 5 & 1.04 & 4 & 1.44 & 4 & 1.67 & 2 & 2.61 & 6 & 3.09 & 4 & 3.83 & 6 & 5.19\\
\cellcolor{gray!6}{luwak} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.08}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.12} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.21}\\
ninja & \textbf{3} & 0.23 & \textbf{3} & 0.35 & \textbf{3} & 0.19 & \textbf{3} & \textbf{0.15} & \textbf{3} & 0.20 & \textbf{3} & 0.17 & \textbf{3} & 0.21 & \textbf{3} & 0.18 & \textbf{3} & 0.19 & \textbf{3} & 0.25 & \textbf{3} & 0.30 & \textbf{3} & 0.33\\
\cellcolor{gray!6}{noxy} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.39} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{\textbf{0.16}} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.23} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{\textbf{0.16}} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.19} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.24} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.30} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.37}\\
orbit & 5 & \textbf{0.22} & 5 & 0.35 & \textbf{6} & 0.26 & 3 & 0.27 & 5 & 0.35 & 3 & 0.43 & 3 & 0.56 & 2 & 0.65 & 3 & 0.77 & 2 & 0.99 & 1 & 1.28 & 2 & 1.50\\
\cellcolor{gray!6}{oryx} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{\textbf{0.09}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.15} & \cellcolor{gray!6}{\textbf{2}} & \cellcolor{gray!6}{0.10} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.26} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.31} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{0.41} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.48} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.58}\\
riptide & \textbf{2} & 0.12 & \textbf{2} & 0.19 & 0 & 0.12 & 0 & \textbf{0.11} & 1 & 0.15 & 0 & 0.16 & 0 & 0.20 & 0 & 0.21 & 1 & 0.29 & 0 & 0.33 & 0 & 0.26 & 0 & 0.31\\
\cellcolor{gray!6}{rxjava2-extras} & \cellcolor{gray!6}{\textbf{3}} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.35} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{\textbf{0.21}} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.27} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.30} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.39} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.41} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.50} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.65} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{0.87} & \cellcolor{gray!6}{2} & \cellcolor{gray!6}{0.95}\\
spring-boot & - & - & \textbf{1} & 1.69 & 0 & 1.02 & \textbf{1} & \textbf{0.73} & \textbf{1} & 0.97 & \textbf{1} & 0.80 & \textbf{1} & 0.98 & \textbf{1} & 0.77 & 0 & 0.90 & 0 & 1.25 & \textbf{1} & 1.46 & 0 & 2.00\\
\cellcolor{gray!6}{timely} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.22} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.33} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.17} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{\textbf{0.12}} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.14} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.18} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.20} & \cellcolor{gray!6}{\textbf{4}} & \cellcolor{gray!6}{0.23}\\
undertow & - & - & 1 & 0.52 & 0 & 0.29 & 0 & \textbf{0.23} & 0 & 0.30 & 1 & 0.25 & 0 & 0.33 & 0 & 0.30 & 0 & 0.36 & 1 & 0.46 & 0 & 0.58 & \textbf{2} & 0.68\\
\cellcolor{gray!6}{wildfly} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{\textbf{40}} & \cellcolor{gray!6}{5.80} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{-} & \cellcolor{gray!6}{1} & \cellcolor{gray!6}{3.74} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{3.01} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{3.81} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{\textbf{2.86}} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{3.32} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{4.35} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{5.38} & \cellcolor{gray!6}{0} & \cellcolor{gray!6}{6.58}\\
wro4j & - & - & - & - & - & - & - & - & 8 & 1.27 & \textbf{9} & 0.91 & 8 & 1.20 & 7 & \textbf{0.83} & 6 & 0.93 & 7 & 1.27 & 6 & 1.22 & 7 & 1.44\\
\cellcolor{gray!6}{yawp} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{\textbf{0.06}} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{\textbf{0.06}} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.08} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.07} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.09} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.11} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.13} & \cellcolor{gray!6}{\textbf{1}} & \cellcolor{gray!6}{0.16}\\
zxing & \textbf{2} & 0.67 & \textbf{2} & 0.90 & \textbf{2} & 0.50 & \textbf{2} & \textbf{0.38} & \textbf{2} & 0.49 & \textbf{2} & \textbf{0.38} & \textbf{2} & 0.49 & \textbf{2} & 0.56 & \textbf{2} & 0.66 & \textbf{2} & 0.86 & \textbf{2} & 1.12 & \textbf{2} & 1.32\\
\bottomrule
\end{tabular}
